Calculating Connection vs. Risk: Understanding How Youth Negotiate Digital Privacy and Security with Peers Online

Youth, while tech-savvy and highly active on social media, are still vulnerable to online privacy and security risks. Therefore, it is critical to understand how they negotiate and manage social connections versus protecting themselves in online contexts. In this work, we conducted a thematic analysis of 1,318 private conversations on Instagram from 149 youth aged 13-21 to understand the digital privacy and security topics they discussed, if and how they engaged in risky privacy behaviors, and how they balanced the benefits and risks (i.e., privacy calculus) of making these decisions. Overall, youth were forthcoming when broaching a wide range of topics on digital privacy and security, ranging from password management and account access challenges to shared experiences of being victims of privacy risks. However, they also openly engaged in risky behaviors, such as sharing personal account information with peers and even perpetrating privacy and security risks against others. Nonetheless, we found many of these behaviors could be explained by the unique "privacy calculus" of youth, where they often prioritized social benefits over potential risks; for instance, youth often shared account credentials with peers to foster social connection and affirmation. As such, we provide a nuanced understanding of youth decision-making regarding digital security and privacy, highlighting both positive behaviors, tensions, and points of concern. We encourage future research to continue to challenge the potentially untrue narratives regarding youth and their digital privacy and security to unpack the nuance of their privacy calculus that may differ from that of adults.

==> Introduction.tex <==

% In the present day, social media platforms, online gaming, and a variety of other digital communication tools have reshaped the way youth interact and express themselves. In fact, much of their social life now takes place online and is mediated by the internet \cite{boyd2008youth}. This digital landscape can prove both empowering \cite{wong_hidden_2020} and challenging \cite{prievara_problematic_2019}. While some have assumed that being immersed in online technologies \cite{gottfried_teens_2023, atske_about_2021} makes youth more tech savvy than the adult population \cite{bennett_digital_2008}, scholars point out that they are a particularly vulnerable demographic who engage in a variety of risky behaviors~\cite{subramaniam2020examining, razi2022instagram}, such as watching inappropriate content \cite{stevens_digital_2019}, receiving unwanted sexual solicitation \cite{drageset_social_2021, tanni_lgbtq_2024} or sexting with strangers \cite{razi_Sext_2020, madigan_prevalence_2018}. In fact, scholars often point out a privacy paradox where youth overshare and engage in risky online behaviors despite the privacy and safety implications of doing so \cite{barnes_privacy_2006, hargittai_what_2016}. Thus, a more nuanced understanding of the ways in which youth engage online and manage their privacy is critical \cite{hodkinson2017bedrooms}. 
\section{Introduction}
In today’s digital age, social media platforms, online gaming, and various other digital communication tools have transformed how youth interact and express themselves. Much of their social life now unfolds online, mediated by the internet \cite{boyd2008youth}. This digital landscape can be both empowering \cite{wong_hidden_2020} and challenging \cite{prievara_problematic_2019}. While some assume that immersion in online technologies \cite{gottfried_teens_2023, atske_about_2021} makes youth more tech-savvy than the adult population \cite{bennett_digital_2008}, scholars argue that they remain a particularly vulnerable demographic, frequently engaging in various risky behaviors~\cite{subramaniam2020examining, razi2022instagram}, such as viewing inappropriate content \cite{stevens_digital_2019}, encountering unwanted sexual solicitation \cite{drageset_social_2021, tanni_lgbtq_2024}, or sexting with strangers \cite{razi_Sext_2020, madigan_prevalence_2018}. Scholars often highlight a “privacy paradox,” in which youth overshare and engage in risky online behaviors despite potential privacy and safety risks \cite{barnes_privacy_2006, hargittai_what_2016}. Consequently, a more nuanced understanding of how youth engage online and manage their privacy is essential \cite{hodkinson2017bedrooms}.
    
% Prior work has focused on youth's individual level of awareness about privacy and security \cite{katavic2023digital}, as well as how to increase awareness through various interventions \cite{quayyum2021cybersecurity}. While youth are cautious about protecting their data privacy, especially on social media, they often lack comprehensive knowledge about digital privacy protection. However, they do express a strong desire for more education on digital privacy \cite{katavic2023digital}. Acknowledging the importance of youth's education, researchers have called for more targeted interventions to effectively increase youth awareness of digital privacy and security issues. Such findings come from interviews and surveys which require reflection on past behavior. These methods can be affected by recall bias ~\cite{raphael1987recall} and may not reflect actual behaviors given the commonly acknowledged gap between stated privacy attitudes and actual privacy behaviors \cite{barnes_privacy_2006}.

% Prior work has primarily examined youth's individual awareness of privacy and security \cite{katavic2023digital} and explored various parental mediation strategies \cite{ghosh2020circle, hashish_involving_2014, akter_from_2022} and educational programs \cite{chattopadhyay2019novel, zhang2017engaging, baciu2019adventures, katavic2023digital} aimed at increasing their awareness \cite{quayyum2021cybersecurity}. However, a significant body of networked privacy research \cite{zhang_privacy_2016, akter_evaluating_2023, rashidi_Android_2018, Lin_expectation_2012, liu_understanding_2019} demonstrated how knowledge and influence from social circles help adult individuals improve their privacy and security awareness and behaviors. Individuals often ask questions and guidance from their close network and learn from the informal stories they hear from others \cite{redmiles2016think, mendel2017susceptibility, das_effect_2014, das_role_2015}. However, when it comes to youth population, we know little about how they engage in discussion about privacy and security when they interact with their peers. As nearly half US teens reported that they are constantly online, and seven in ten said they use a social media platform everyday \cite{noauthor_teens_2024}, it is important to know when they interact with their peers online how they exchange their informal stories about privacy and security in general. Ironically, young generations are often more tech savvy than their older counterparts \cite{works_you_2019, akter_it_2023, correa_brokering_2015}. This body of existing research creates an interesting opportunity to explore whether youth themselves, being techsavvy generations, engage in risky privacy and security behavior and potentiually digital harm to others, and if they do so, what potential benefits motivate them in participating in risks and sharing the incidences with others.   
Prior research has primarily focused on youth's individual awareness of privacy and security \cite{katavic2023digital} and examined various parental mediation strategies \cite{ghosh_circle_2020, hashish_involving_2014, akter_from_2022} as well as educational programs \cite{chattopadhyay2019novel, zhang2017engaging, baciu2019adventures, katavic2023digital} aimed at increasing their awareness \cite{quayyum2021cybersecurity}. However, a significant body of networked privacy research \cite{zhang_privacy_2016, akter_evaluating_2023, rashidi_Android_2018, Lin_expectation_2012, liu_understanding_2019} has demonstrated that knowledge and influence from social circles can play a crucial role in helping adult individuals improve their privacy and security awareness and behaviors - individuals frequently seek guidance from their close networks and learn from the informal stories shared within these circles \cite{redmiles2016think, mendel2017susceptibility, das_effect_2014, das_role_2015}.

In contrast, there is limited knowledge about how youth discuss privacy and security when interacting with their peers. Given that nearly half of U.S. teens report being constantly online, and seven in ten use social media platforms daily \cite{noauthor_teens_2024}, it is essential to understand how they exchange informal stories about privacy and security with their peers in these digital spaces. This body of existing research creates an interesting opportunity to explore whether youth themselves, as a tech-savvy generation \cite{works_you_2019, akter_it_2023, correa_brokering_2015}, engage in risky privacy and security behaviors and potentially are conduits of digital harm to others. Furthermore, to design support systems for youth, it is crucial to explore what motivates them to participate in such risks and share these incidents with peers.

% The paradoxical nature of families and society wanting to increase youth's digital privacy and security, while youth are more likely to be on social media and have more knowledge about technology, creates an interesting opportunity to explore how they discuss their privacy and security stories with their peers, and whether 


% design collaborative technologies where parents and teens could potentially support one another in accomplishing the shared goal of mobile online safety and privacy management within families. 

%  half of them are "almost constantly" online. 


% youth are constantly online and use social media, it is important to know how they exchange their informal stories about privacy and security with their peers online. Moreover, as youth are techsavvy generation in general, we also want to know whether they engage in risky behaviors, and what motivates them to do so. 


% However, networked privacy researchers have called for adopting more community-based approaches rather than individual ones to effectively manage privacy and security. This is because, individuals often ask questions and guidance regarding digital privacy and security from their social circles. They often get influenced to change their privacy behavior by their social network. But they primarilly focused on adult individuals and we have little knowledge about how youth population does so from their peers. Additionally, being techsavvy, we also need to know whether the youth themselves get engaged in risky behavior by themselves. Apart from this, we find it important to explore their motivation behind this risky behaviors. 




% Although youth tend to be cautious about protecting their data privacy, especially on social media, they often lack a comprehensive understanding of digital privacy protections. However, many express a strong desire for more education on digital privacy \cite{katavic2023digital}. Recognizing the importance of educating youth, researchers have advocated for more targeted interventions to effectively raise awareness of digital privacy and security issues. These findings are largely based on interviews and surveys, which require participants to reflect on past behaviors. Such methods can be affected by recall bias ~\cite{raphael1987recall} and may not accurately represent actual behaviors, given the well-documented gap between stated privacy attitudes and actual practices \cite{barnes_privacy_2006}.
   
% Analyzing digital trace data, such as private conversations, offers a way that such biases can be reduced, while also providing information on a distinct dynamic of youth online interaction. Thus, to better understand the privacy attitudes and behaviors of youth, we examined youth private social media interactions with peers. We focused on conversations having to do with security and privacy. This provided an unobtrusive means of understanding youth online behaviors, perspectives, and struggles with security and privacy. Specifically, we were guided by the following research questions: 
Prior research \cite{razi_Sext_2020, hartikainen2021safe, prescott2017peer} demonstrates that analyzing digital trace data, such as private conversations, provides an opportunity to capture the unique dynamics of youth online interactions. To gain a deep understanding of youth privacy attitudes and behaviors, we examined private social media interactions among youth and their peers, focusing on conversations related to security and privacy. This approach offered an \edit{naturalistic} way to observe youth perspectives, online behaviors, and challenges with privacy and security. 
Finally, we examined youth risk behavior related to privacy and security through the lens of privacy calculus in order to capture their unique process of risk-taking behavior. Privacy calculus is a prominent framework for understanding how individuals weigh the benefits and the risks associated with their behavior. \edit{Overall, our study aims to understand the experiences of digital privacy and security among youth and how they negotiate these issues with peers online. We investigated how youth navigate social connections versus protecting themselves in online contexts. } Our study was guided by the following research questions:



\begin{itemize}
\item \textbf{RQ1:} \textit{How do youth share and discuss their privacy and security experiences in private online chats?}  
    
\item \textbf{RQ2:} \textit{How do youth participate in risky behaviors regarding their digital privacy and security in private online chats?}

\item \textbf{RQ3:} \textit{How do youth weigh the risks against benefits of risky privacy and security behaviors?} 

\end{itemize}

% In order to address these research questions, we leveraged Instagram private conversations (i.e., Direct Messages, DMs) that US youth ages 13-21 took part in. The conversation data was donated by youth as part of the Instagram Data Donation Project (IGDD) \cite{razi2022instagram}. This dataset provides access to youth personal online discussions on security and privacy topics with others. We used a set of privacy and security related keywords identified in prior research~\cite{wisniewski2018privacy, kumar2023understanding} to retrieve initial conversation data. Then, we manually reviewed the data to sort relevant discussions within this dataset. From this curated dataset of 1,318 conversations, a thematic analysis~\cite{braun2006using} was performed to identify significant trends within the database. 
Overall, our research questions focus on how youth discuss privacy risks, participate in risky behaviors, and weigh risks against benefits in their decision-making. To address these research questions, we conducted a study with youth participants aged 13 to 21. Using a custom web-based system, participants securely uploaded their private Instagram conversations.
% we analyzed Instagram private conversations (i.e., Direct Messages, or DMs) involving U.S. youth aged 13-21. The conversation data was contributed by youth participants as part of the \textcolor{red}{Instagram Data Donation Project (IGDD) \cite{razi2022instagram}}. 
This conversation dataset provided valuable insights into youth's personal online discussions on security and privacy topics. We used a set of privacy- and security-related keywords identified in prior research~\cite{wisniewski2018privacy, kumar2023understanding} to initially retrieve conversation data. Subsequently, we reviewed and sorted relevant discussions within this dataset. From the curated set of 1,318 conversations, we conducted a thematic analysis~\cite{braun2006using} to identify the themes. 


% \textcolor{red}{Need a paragraph here summarizing the themes from RQ1 and RQ2}
% Overall, we found that youth most frequently discussed potential privacy and security threats that they identified on time, and what protective measures they took to safeguard against those threats (RQ1). They also often disclosed their password management practices and the challenges they experienced related to their account access. However, they often shared stories of themselves being victims of privacy and security risks. Regarding the risky behaviors youth took part in, we found that youth frequently shared sensitive account information with their peers (RQ2). Ironically, they also often shared stories of how they perpetrated security and privacy threats to others. Our analysis further reveals that youth engage in a privacy calculus \cite{wisniewski_privacy_2022} weighing the benefits of social support against the risks of various privacy and security-related behaviors \cite{house_work_1981}. While youth often recognized online security risks of engaging in poor password practices or financial scams, the social benefits sometimes outweighed these risks (R3). For example, youth sometimes shared passwords with peers despite knowing the security risk, which prior work has identified as a way youth create social connection with others through trust \cite{marwick_networked_2014}. We found that youth even broadcast such unsafe behaviors to their peers, which allowed them to receive social affirmation that this was a socially acceptable practice. Clearly, social considerations shaped their privacy and security decisions. 
\edit{Through a thematic analysis of private social media conversations (Instagram), we identified the topics discussed and examined how youth address privacy and online risks. Our results also highlighted risky behaviors, such as sharing personal information and perpetuating privacy and security risks against others.} Our findings revealed that youth frequently discussed the potential privacy and security threats they identified in a timely manner and shared the protective measures they took to safeguard themselves against those threats (RQ1). They also commonly disclosed their password management practices and the challenges they faced related to account access. Furthermore, youth often shared their personal experiences of falling victim to privacy and security risks themselves. Regarding their own risky behaviors, we found that youth frequently shared sensitive account information, especially login credentials, with peers (RQ2). Ironically, they also recounted instances in which they themselves perpetrated security and privacy threats, such as hacking, spamming, or scamming others.

Our analysis further revealed that youth engaged in a privacy calculus, \cite{wisniewski_privacy_2022} weighing the benefits of social support against the risks of various privacy and security-related behaviors \cite{house_work_1981} (RQ3). While youth often recognized the online security risks of engaging in poor password practices or financial scams, the social benefits sometimes outweighed these risks. For example, youth often shared passwords with peers despite knowing the security risk, which prior work has identified as a way youth create a social connection with others through trust \cite{marwick_networked_2014}. Moreover, youth often broadcast these unsafe practices to their peers, receiving social affirmation that reinforced the acceptability of these behaviors, underscoring the significant role of social considerations in shaping their privacy and security decisions. We also observed that this privacy calculus was at the root of a disconcerting trend: youth discussed how they planned to or had already carried out privacy and security attacks on others. In these cases, a desire for peer affirmation of the attack overshadowed doubts about violating others' privacy and security. Consequently, the need for social support, coupled with peers' willingness to endorse such actions, emerged as an unanticipated outcome of youths' privacy calculus.

% Overall, our study expands on the existing knowledge in CSCW by shifting from youth's individual digital privacy awareness to the peer-driven dynamics that shape their behavior. Unlike previous research focused on educational programs or parental mediation technologies, our work uniquely examines when youth discuss privacy and security matters with their online peers, how they share their risk experiences, whether they position themselves as victims or perpetrators, and what motivates these interactions. Through a thematic analysis of their private Instagram conversations, we revealed the nuanced role of peer influence in youth's navigation of digital privacy and security risks, enriching the literature on social support in networked privacy. Our findings offer actionable insights for designers, advocating for features like controlled account-sharing, enhanced privacy alerts, and automated scam detection to balance privacy with social connection. Additionally, education-focused design elements can guide youth toward responsible privacy management, leveraging peer support as a motivator. 
% \edit{ The dataset of 1,318 private conversations provides a promising foundation for investigating a critical topic for CSCW audiences. }

\edit{Overall, our study extends the existing knowledge in CSCW by shifting the focus from individual digital privacy awareness to the peer-driven dynamics that shape youth behavior. Unlike previous work centered on educational programs or parental mediation, our analysis of private Instagram conversations provides a promising foundation for investigating a critical topic for CSCW audiences. The emphasis on peer influence and real-world conversation data makes our work particularly relevant to understanding youth online behavior. In sum, our study highlighted how youth navigate digital privacy and security in peer interactions on Instagram, using the "privacy calculus" framework to analyze their decision-making.
% highlights when and how youth discuss privacy risks, the roles they assume in these discussions, and the motivations behind their interactions. 
Our findings offer insights for designing features such as controlled account-sharing, enhanced privacy alerts, and automated scam detection to balance privacy with social connection. Additionally, education-focused design elements can leverage peer support to promote responsible privacy management.}
In summary, our study makes the following contribution to the CSCW research community: 
% Based on our findings, we provide implications for design and education to promote positive online privacy and security practices for youth. As such, we make the following contribution to the CSCW community:

\begin{itemize}
    \item A comprehensive analysis of youth private conversations with their peers regarding their online security and privacy practices.
    \item An understanding of the social dynamics that drive decision-making related to their disclosures of security and privacy risk exposures and their own risky behaviors. 
    \item Design recommendations for further steps to help mitigate youth participation in risky security and privacy practices, while allowing them to maintain social bonding with their peers.
\end{itemize}
